Learning Multi-View Aggregation In the Wild for Large-Scale 3D Semantic Segmentation

Recent works on 3D semantic segmentation propose to exploit the synergy between images and point clouds by processing each modality with a dedicated network and projecting learned 2D features onto 3D points. Merging large-scale point clouds and images raises several challenges, such as constructing a mapping between points and pixels, and aggregating features between multiple views. Current methods require mesh reconstruction or specialized sensors to recover occlusions, and use heuristics to select and aggregate available images. In contrast, we propose an end-to-end trainable multi-view aggregation model leveraging the viewing conditions of 3D points to merge features from images taken at arbitrary positions. Our method can combine standard 2D and 3D networks and outperforms both 3D models operating on colorized point clouds and hybrid 2D/3D networks without requiring colorization, meshing, or true depth maps. We set a new state-of-the-art for large-scale indoor/outdoor semantic segmentation on S3DIS (74.7 mIoU 6-Fold) and on KITTI-360 (58.3 mIoU). Our full pipeline is accessible at https://github.com/drprojects/DeepViewAgg, and only requires raw 3D scans and a set of images and poses.

==> figures/viewing.tex <==
\begin{tabular}{cc}
    
    \includegraphics[width=.4\linewidth, height=.13\textheight]{figures/modules/images/image_0_star.png}
     &
    \begin{tikzpicture}
    \begin{axis}[
    	xlabel=Group1,
    	xtick={0,0.5,1},
    	ytick={0.5,0},
    	grid=major,
    	xmin=0, xmax=1,
        ymin=0, ymax=1,
	    width =.55\linewidth,
		height=.15\textheight]
        \addplot[color=red,mark=x] coordinates {
    	(0,    0.5)
    	(1,   0.4)
        };
        \addplot[color=blue,mark=*] coordinates {
    	(0,    0.3)
    	(1,   0.2)
        };
    \end{axis}
    \end{tikzpicture}
    \\
       \begin{tikzpicture}
    \begin{axis}[
    	xlabel=Group2,
    	xtick={0,0.5,1},
    	ytick={0},
    	xmin=0, xmax=1,
        ymin=0, ymax=1,
        grid=major,
	    width =.55\linewidth,
		height=.15\textheight]
        \addplot[color=red,mark=x] coordinates {
    	(0,    0.5)
    	(1,   0.4)
        };
        \addplot[color=blue,mark=*] coordinates {
    	(0,    0.3)
    	(1,   0.2)
        };
    \end{axis}
    \end{tikzpicture}
    &
       \begin{tikzpicture}
    \begin{axis}[
    	xlabel=Group3,
    	xtick={0,0.5,1},
    	ytick={0.5,0},
    	xmin=0, xmax=1,
        ymin=0, ymax=1,
        grid=major,
	    width =.55\linewidth,
		height=.15\textheight]
        \addplot[color=red,mark=x] coordinates {
    	(0,    0.5)
    	(1,   0.4)
        };
        \addplot[color=blue,mark=*] coordinates {
    	(0,    0.3)
    	(1,   0.2)
        };
    \end{axis}
    \end{tikzpicture} \\
    \multicolumn{2}{c}{
    \begin{tabular}{rlrl}
        \begin{tikzpicture}
        \draw[draw=none, very thick, mark=o] (0,0) -- (0,0);
        \draw[draw=blue, very thick] (0,0.1) -- (1,0.1);
        \filldraw [blue] (0.5,0.1) circle (3pt);
        %\node at (0.5,0.2) {\pgfuseplotmark{o}};
        \end{tikzpicture}
         &
         distance
         & 
         \begin{tikzpicture}[baseline=-1mm]
        %\draw[draw=none, very thick, mark=o] (0,0) -- (0,0);
        \draw[draw=red, very thick] (0,-0) -- (1,-0);
        \node[red, scale=1, thick, scale=2] at (0.5,-0) {\pgfuseplotmark{x}};
        \end{tikzpicture}
         &
         angle
    \end{tabular}
    }
      
        
\end{tabular}
